A dynamic programming approach for distributing quantum circuits by bipartite graphs

Near-term large quantum computers are not able to operate as a single processing unit. It is therefore required to partition a quantum circuit into smaller parts, and then each part is executed on a small unit. This approach is known as distributed quantum computation. In this study, a dynamic programming algorithm is proposed to minimize the number of communications in a distributed quantum circuit (DQC). This algorithm consists of two steps: first, the quantum circuit is converted into a bipartite graph model, and then a dynamic programming approach (DP) is proposed to partition the model into low-capacity quantum circuits. The proposed approach is evaluated on some benchmark quantum circuits with remarkable reduction in the number of required teleportations.

==> QFTT.tex <==

\centering
\begin{tabular}{|c|c|c|c|}
\hline
 n & K&Number of teleportation&partitions\\
\hline
6&2&5&\{\ket{q_{1}}\}\{\ket{q_{2}},\ket{q_{3}},\ket{q_{4}},\ket{q_{5}},\ket{q_{6}}\}\\
\hline
6&3&9&\{\ket{q_{1}}\}\{\ket{q_{2}}\}\{\ket{q_{3}},\ket{q_{4}},\ket{q_{5}},\ket{q_{6}}\}\\
\hline
6&4&12&\{\ket{q_{1}}\}\{\ket{q_{2}}\}\{\ket{q_{3}}\},\{\ket{q_{5}},\ket{q_{6}}\}\\
\hline
7&2&6&\{\ket{q_{1}}\}\{\ket{q_{2}},\ket{q_{3}},\ket{q_{4}},\ket{q_{5}},\ket{q_{6}},,\ket{q_{7}}\}\\

\hline
\end{tabular}
